REAPS: Towards Better Recognition of Fine-grained Images by Region Attending and Part Sequencing

Fine-grained image recognition has been a hot research topic in computer vision due to its various applications. The-state-of-the-art is the part/region-based approaches that first localize discriminative parts/regions, and then learn their fine-grained features. However, these approaches have some inherent drawbacks: 1) the discriminative feature representation of an object is prone to be disturbed by complicated background; 2) it is unreasonable and inflexible to fix the number of salient parts, because the intended parts may be unavailable under certain circumstances due to occlusion or incompleteness, and 3) the spatial correlation among different salient parts has not been thoroughly exploited (if not completely neglected). To overcome these drawbacks, in this paper we propose a new, simple yet robust method by building part sequence model on the attended object region. Concretely, we first try to alleviate the background effect by using a region attention mechanism to generate the attended region from the original image. Then, instead of localizing different salient parts and extracting their features separately, we learn the part representation implicitly by applying a mapping function on the serialized features of the object. Finally, we combine the region attending network and the part sequence learning network into a unified framework that can be trained end-to-end with only image-level labels. Our extensive experiments on three fine-grained benchmarks show that the proposed method achieves the state of the art performance.

==> sections/PRCV_4_experiments.tex <==

\section{Performance Evaluation}
\label{others}

\subsection{Datasets and Implementation Details}

We conduct experiments on three benchmark datasets, including Stanford Cars~\cite{krause2015fine}, FGVC-aircraft~\cite{maji2013fine} and CUB-200-2011~\cite{WahCUB_200_2011}, which are widely used to evaluate fine-grained image recognition. Table~\ref{dataset} shows the detailed statistics of the three datasets.
%
\begin{table}
  \caption{Statistics of three fine-grained benchmark datasets used in this paper.}
  \label{dataset}
  \centering
  \begin{tabular}{llll}
    \toprule
    Dataset          &  Category     &  Training     &  Testing\\
    \midrule
    Stanford Cars~\cite{krause2015fine} & 196           & 8,144         & 8,041   \\
    FGVC-aircraft~\cite{maji2013fine} & 100           & 6,667         & 3,333   \\
    CUB-200-2011~\cite{WahCUB_200_2011}  & 200           & 5,994         & 5,794   \\
    \bottomrule
  \end{tabular}
\end{table}
%
For fair comparison, all compared methods employ similar backbone network. Specifically, we start with the 19-layer VGGNets pre-trained on ImageNet and fine-tune it on the three fine-grained datasets. The parameters of RAN and PSN are initialized with the same pre-trained model. Input images and the cropped attended regions are both resized to $448\times448$, where high resolution highlights details and benefits recognition. We use SGD with momentum 0.9 to minimize the loss function $\mathcal{L}$ in Eq.~(\ref{loss_function}), where $\lambda_1$, $\lambda_2$, and $\lambda_3$ are all set to 1. The threshold $\tau$ in Eq.~(\ref{cam_op}) is set to $0.1$. Following the common practice of learning rate decaying schedule, the initial learning rate is set to 0.001 and multiplied by 0.1 every 60 epoches.

\subsection{Results on Stanford Cars}

%{\color{red}
\paragraph{Effectiveness of part branch in PSN.}
As pointed out in Section~\ref{sec_part_model}, we take LSTM as the mapping function to map the serialized features to discriminative part representation, instead of learning part extractors explicitly.
%It is supposed that LSTM is able to enhance the discriminative capacity of local feature with the prior knowledge of object structure.
To evaluate the effectiveness of the LSTM-based part learning branch, we present the classification results of two models: \emph{PSN wo/w part}, which are based on the $P_g$ \emph{without/ with} the part modeling branch. The results are shown in Table~\ref{lstm-part-table}. We can see that the model adopting part sequence modeling branch achieves a relative performance gain of 1.5\%. Some illustrations are given in Figure~\ref{lstm-part-fig}.
%By multi-task training with both global pooling branch and part sequence learning branch, the shared backbone network benefits from the complementary information between global and part representation, thus it can focus on more salient parts, enrich finer details of the object and ignore the irrelevant regions.
 It can be observed that the part branch encourages a more compact distribution on the feature maps, further enhances the crucial part areas and depresses the unless ones. Moreover, since we do not fix the number of parts, the LSTM-based part learning branch is able to judge and localize discriminative parts {\color{red}initiatively}. In summary, as expected the part branch focuses on the discriminative parts and generates mapped representation in a more flexible and robust way.
%}

\begin{table}
  \caption{Effectiveness of part sequence modeling branch in PSN.}
  \label{lstm-part-table}
  \centering
  \begin{tabular}{cc}
    \toprule
    Approach                     &  Accuracy\\
    \midrule
    PSN wo part        &  88.3        \\
    PSN w part        &  89.8        \\
    %REAL wo part      &  91.7        \\
    %REAL w part      &  92.6        \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{images/lstm_feature_map.pdf}
  \caption{Feature maps of some examples from (a) Stanford Cars, (b) FGVC Aircraft, (c) CUB-200-2011. From left to right in (a-c), the pictures are the raw image, the feature map generated by PSN without part branch, and the feature map generated by PSN with part branch, respectively.}
  \label{lstm-part-fig}
\end{figure}


\paragraph{Effectiveness of region attending network.} We first visualize some results of our CAM-based region attending network in Fig.~\ref{region-atten-fig} for qualitative analysis. The discriminative regions of the input images are highlighted. The attended regions that are cropped from the raw images and then amplified preserve the object-level structures, eliminate background interference and enrich the local visual details.
As the attending process is ``self-guided'' and requires no bounding box or part annotation, we then evaluate its effectiveness by classification accuracy. In Table~\ref{region-atten-table}, we compare the result of our PSN with that of two other attention based approaches. To be fair, we select the single-attention based performance from FCAN~\cite{liu2016fully} and the second scale result from RA-CNN~\cite{fu2017look}. RA-CNN\cite{fu2017look} is the most relevant work to ours in terms of the region attention concept and the way to use it. We can see that our method outperforms FCAN~\cite{liu2016fully} with a clear margin (6.7\% relative gain) and RA-CNN\cite{fu2017look} with 0.9\% accuracy improvement. In addition, our approach can be trained end-to-end. All the above shows the superior attention localization ability of our method.

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{images/attended_region.pdf}
  \caption{Region attention localization results at the second scale for some examples from (a) Stanford Cars, (b) FGVC-aircraft, and (c) CUB-200-2011. From left to right in (a-c), the pictures are the raw image, the attention mask with bounding box indicating the area of top attention response, and the cropped object-level region, respectively.}
  \label{region-atten-fig}
\end{figure}

\begin{table}
  \caption{Performance comparison of attention localization on the Stanford Cars dataset.}
  \label{region-atten-table}
  \centering
  \begin{tabular}{cc}
    \toprule
    Approach                                        &  Accuracy\\
    \midrule
    FCAN (single-attention)~\cite{liu2016fully}      &  84.2    \\
    RA-CNN (scale 2)~\cite{fu2017look}               &  90.0    \\
    PSN                                   &  90.9    \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Effectiveness of fine-grained recognition.} We compare our REAPS with several existing methods, the results are summarized in Table~\ref{car-accuracy}. Our method achieves better performance than PA-CNN~\cite{krause2015fine} that uses bounding box annotations in both training and testing, and outperforms Improved B-CNN~\cite{lin2017improved}, BoostCNN~\cite{moghimi2016boosted} and KP~\cite{cui2017kernel} that use very high-dimensional feature representations. Both FCAN~\cite{liu2016fully} and RA-CNN~\cite{fu2017look} boost representation learning via region attention recurrently, in comparison with them our approach achieves better accuracy by 2.5\% and 0.5\% improvement due to accurate attention localization and part sequence modeling. With a much smaller network and much simpler end-to-end training process, our approach also surpasses MA-CNN~\cite{zheng2017learning} that employs five independent VGG-19 to extract features of four parts and the whole object.

\begin{table}
  \caption{Performance comparison on the Stanford Cars dataset. \emph{Train Anno}. indicates whether bounding box or part annotation is used in training.}
  \label{car-accuracy}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Approach                     &  Train Anno.       &  Accuracy\\
    \midrule
    MDTP~\cite{wang2016mining}                         &  \Checkmark        &  92.5    \\
    PA-CNN~\cite{krause2015fine}                       &  \Checkmark        &  92.8    \\
    FCAN~\cite{liu2016fully}                           &                    &  91.5    \\
    Improved B-CNN~\cite{lin2017improved}              &                    &  92.0    \\
    BoostCNN~\cite{moghimi2016boosted}                 &                    &  92.1    \\
    KP~\cite{cui2017kernel}                            &                    &  92.4    \\
    RA-CNN (scale 1+2+3)~\cite{fu2017look}             &                    &  92.5    \\
    MA-CNN (4 parts + object)~\cite{zheng2017learning} &                    &  92.8    \\
    \midrule
    %xxx (scale 2)                                     &                    &  90.9    \\
    REAPS                                   &                    &  93.0    \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Results on FGVC-aircraft}

The results on FGVC-aircraft are summarized in Table~\ref{aircraft-accuracy}. Since aircraft bears strong sequence property, our REAPS outperforms all the compared methods, which shows the effectiveness of our attention localization and part sequence modeling. Concretely, REAPS obtains the best accuracy of 91.6\%, surpassing MA-CNN~\cite{zheng2017learning} by a relative 1.7\% gain. The significant improvement suggests that the proposed part sequence modeling network works as expected to leverage spatial information of parts, and does even better when the objects to be recognized have strong sequential structures.

\begin{table}
  \caption{Performance comparison on the FGVC-aircraft dataset. \emph{Train Anno}. indicates whether bounding box or part annotation is used in training.}
  \label{aircraft-accuracy}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Approach                     &  Train Anno.       &  Accuracy\\
    \midrule
    MG-CNN~\cite{wang2015multiple}                     &  \Checkmark        &  86.6    \\
    MDTP~\cite{wang2016mining}                         &  \Checkmark        &  88.4    \\
    KP~\cite{cui2017kernel}                            &                    &  86.9    \\
    RA-CNN (scale 1+2+3)~\cite{fu2017look}             &                    &  88.2    \\
    Improved B-CNN~\cite{lin2017improved}              &                    &  88.5    \\
    BoostCNN~\cite{moghimi2016boosted}                 &                    &  88.5    \\
    MA-CNN (4 parts + object)~\cite{zheng2017learning} &                    &  89.9    \\
    \midrule
    %xxx (scale 2)                                     &                    &  90.1    \\
    REAPS                                   &                    &  91.6    \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Results on CUB-200-2011}

The results on CUB-200-2011 are summarized in Table~\ref{bird-accuracy}. Thanks to accurate attention localization and part sequence modeling, REAPS achieves better performance than RA-CNN(scale 1+2+3)~\cite{fu2017look} that is the most related work to ours by a relative gain of 0.7\%, and surpasses PA-CNN~\cite{branson2014bird} and Mask-CNN~\cite{wei2016mask}, all of which turn to extra annotations for help. B-CNN-based methods~\cite{lin2017improved, moghimi2016boosted, cui2017kernel} show outstanding performance on fine-grained classification task by high-dimensional feature representation, and comparing with them, our method obtains comparable performance. Furthermore, we incorporate one more PSN into our framework, and the 2nd PSN is based on the attended region of the 1st PSN. We denote the resulting network REAPS+. We can see that REAPS+ obtains the highest accuracy of 86.8\%, surpassing the corresponding RA-CNN(scale 1+2+3)~\cite{fu2017look} by 1.5\% improvement and MA-CNN~\cite{zheng2017learning} that employs 6 independent VGG-19 to extract features for the four attended parts, the object region and the raw image.

\begin{table}
  \caption{Performance comparison on the CUB-200-2011 dataset. \emph{Train Anno}. indicates whether bounding box or part annotation is used in training.}
  \label{bird-accuracy}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Approach                     &  Train Anno.       &  Accuracy\\
    \midrule
    PA-CNN~\cite{krause2015fine}                       &  \Checkmark        &  82.8    \\
    MG-CNN~\cite{wang2015multiple}                     &  \Checkmark        &  83.0    \\
    PN-CNN~\cite{branson2014bird}                      &  \Checkmark        &  85.4    \\
    Mask-CNN~\cite{wei2016mask}                        &  \Checkmark        &  85.4    \\
    STNs~\cite{jaderberg2015spatial}                   &                    &  84.1    \\
    FCAN~\cite{liu2016fully}                           &                    &  84.3    \\
    PDFR~\cite{zhang2016picking}                       &                    &  84.5    \\
    RA-CNN (scale 1+2+3)~\cite{fu2017look}             &                    &  85.3    \\
    Improved B-CNN~\cite{lin2017improved}              &                    &  85.8    \\
    BoostCNN~\cite{moghimi2016boosted}                 &                    &  86.2    \\
    KP~\cite{cui2017kernel}                            &                    &  86.2    \\
    MA-CNN (4 parts + object)~\cite{zheng2017learning} &                    &  86.5    \\
    \midrule
    %xxx (scale 2)                                     &                    &  83.2    \\
    %xxx (scale 3)                                     &                    &  83.1    \\
    REAPS                                   &                    &  86.0    \\
    REAPS+                                 &                    &  86.8    \\
    \bottomrule
  \end{tabular}
\end{table}

